DEMO: Relay/Replay Attacks on GNSS signals

Global Navigation Satellite Systems (GNSS) are ubiquitously relied upon for positioning and timing. Detection and prevention of attacks against GNSS have been researched over the last decades, but many of these attacks and countermeasures were evaluated based on simulation. This work contributes to the experimental investigation of GNSS vulnerabilities, implementing a relay/replay attack with off-the-shelf hardware. Operating at the signal level, this attack type is not hindered by cryptographically protected transmissions, such as Galileo's Open Signals Navigation Message Authentication (OS-NMA). The attack we investigate involves two colluding adversaries, relaying signals over large distances, to effectively spoof a GNSS receiver. We demonstrate the attack using off-the-shelf hardware, we investigate the requirements for such successful colluding attacks, and how they can be enhanced, e.g., allowing for finer adversarial control over the victim receiver.

==> Demo Replaying Attacks on GNSS systems_arxiv_only/acronyms.tex <==
%% network protocols
\newacronym{dhcp}{DHCP}{Dynamic Host Configuration Protocol}
\newacronym{ntp}{NTP}{Network Time Protocol}
\newacronym{tcp}{TCP}{Transmission Control Protocol}
\newacronym{udp}{UDP}{User Datagram Protocol}
\newacronym{crc}{CRC}{Cyclic Redundancy Check}

% signal modulation, effects, etc
\newacronym{rss}{RSS}{Received Signal Strength}
\newacronym{mimo}{MIMO}{Multiple Input Multiple Output}
\newacronym{ofdm}{OFDM}{Orthogonal Frequency Division Multiplexing}
\newacronym{dsss}{DSSS}{Direct Sequence Spread Spectrum}
\newacronym{css}{CSS}{Chirp Spread Spectrum}
\newacronym{fsk}{FSK}{Frequency Shift Keying}
\newacronym{snr}{SNR}{Signal-to-Noise Ratio}
\newacronym{sinr}{SINR}{Signal to interference plus noise ratio}
\newacronym{aoa}{AoA}{Angle of Arrival}
\newacronym{ssc}{SSC}{Secret Spreading Code}
\newacronym{ci}{CI}{Constructive Interference}
\newacronym{cfo}{CFO}{Carrier Frequency Offset}
\newacronym{cpo}{CPO}{Carrier Phase Offset}
\newacronym{sf}{SF}{Spreading Factor}


% security
\newacronym{rra}{RRA}{Record-and-Replay-Attack}
\newacronym{dd}{DD}{Distance-Decreasing}
\newacronym{aua}{AuA}{Area under Attack}

% GNSS terms
\newacronym{gnss}{GNSS}{Global Navigation Satellite System}
\newacronym{gps}{GPS}{Global Positioning System}
\newacronym{nmea}{NMEA}{National Marine Electronics Association}
\newacronym{nasa}{NASA}{National Aeronautics and Space Administration}
\newacronym{agps}{A-GPS}{Assisted/Augmented GPS}
\newacronym{scer}{SCER}{Security Code Estimation and Replay}
\newacronym{nma}{OS-NMA}{Open Service Navigation Message Authentication}
\newacronym{sis}{SIS}{Signal In Space}
\newacronym{raim}{RAIM}{Receiver autonomous integrity monitoring}
\newacronym{pvt}{PVT}{Position-Velocity-Time}

% Hardware / Software
\newacronym{sdr}{SDR}{Software Defined Radio}
\newacronym{sdrs}{SDR}{Software Defined Radios}
\newacronym{ots}{OTS}{Off-the-Shelf}
\newacronym{rt}{RT}{Real-Time}
\newacronym{ide}{IDE}{Integrated Development Environment}
\newacronym{fifo}{FIFO}{First-In-First-Out}
\newacronym{sma}{SMA}{SubMiniature Version A}
\newacronym{rf}{RF}{Radio Frequency}

% soft terms
\newacronym{foi}{FoI}{Feature of Interest}


